Vector representations of text data in deep learning

In this dissertation we report results of our research on dense distributed representations of text data. We propose two novel neural models for learning such representations. The first model learns representations at the document level, while the second model learns word-level representations. For document-level representations we propose Binary Paragraph Vector: a neural network models for learning binary representations of text documents, which can be used for fast document retrieval. We provide a thorough evaluation of these models and demonstrate that they outperform the seminal method in the field in the information retrieval task. We also report strong results in transfer learning settings, where our models are trained on a generic text corpus and then used to infer codes for documents from a domain-specific dataset. In contrast to previously proposed approaches, Binary Paragraph Vector models learn embeddings directly from raw text data. For word-level representations we propose Disambiguated Skip-gram: a neural network model for learning multi-sense word embeddings. Representations learned by this model can be used in downstream tasks, like part-of-speech tagging or identification of semantic relations. In the word sense induction task Disambiguated Skip-gram outperforms state-of-the-art models on three out of four benchmarks datasets. Our model has an elegant probabilistic interpretation. Furthermore, unlike previous models of this kind, it is differentiable with respect to all its parameters and can be trained with backpropagation. In addition to quantitative results, we present qualitative evaluation of Disambiguated Skip-gram, including two-dimensional visualisations of selected word-sense embeddings.

==> beyond_dbow.tex <==
\chapter{Beyond distributed bag of words}

WARNING: due to~\cite{li2015learning}, this chapter will probably be removed or merged into chapter \ref{sec:dsh}.

~

In this chapter we propose a simple extension to one of the two neural models introduced in~\cite{le2014distributed}.
As discussed in \sectionref{document_embeddings}, paragraph vector distributed bag of words (PV-DBOW) model
learns paragraph embeddings by predicting all words in a document.
Unlike paragraph vector distributed memory (PV-DM) model,
PV-DBOW does not take context as an input and, therefore, can be considered a weaker model.
In this chapter we describe a simple extension, which attempts to alleviate this weakness.

\section{Distributed bag of n-grams}

Instead of predicting document's words we propose to predict document's n-gram, i.e. subsequences of consecutive words in the document.
We discovered that when predicting all words and all bigrams we get up to 5\% improvement over the unigram model.
Including trigrams to the dictionary does not further improve the performance.

It is good to take all words from dictionary and all bigrams.
However, for big corpora the set of all uni- and bi-grams can be big
and, therefore, the output layer weigh matrix can be to big to fit in the memory.
Therefore, in practice the dictionary should be as big as possible, depending on available memory.
The dictionary can be shrunk by taking only a predefined number of globally most popular n-gram or n-grams
that occur no less than specified number of times in the corpus.

\section{Experiments}

To demonstrate usefulness of our modification we performed experimental evaluation.
In this chapter we confine experiments to sentiment analysis task.
In the next chapter we use this extension to improve information retrieval results.

Sentiment analysis often boils down to binary classification.
Given a set of train examples labeled with either positive or negative sentiment
we train the model to be able to assign test results to one of those two categories.
We replicated experiment described in~\cite[section 3.2]{le2014distributed}.
We trained 400-dimensional PV-DBOW model on 75 thousands training documents from Large Movie Review Dataset~\cite{maas2011learning}.
From those 75 thousands we extracted 25 thousands labeled examples
and we used them to fit a small neural network with 50 hidden and one output neuron,
as the one depicted on~\figref{binary_classification_neural_network}.
%
\begin{figure}[htb!]
  \centering
  \includegraphics[width=0.4\linewidth]{binary_classification_neural_network}
  \longcaption{A simple feedforward neural network used for binary classification.}{There are $ m $ input signals, $ 50 $ hidden neurons
  and just one output neuron. Weights for each neuron are rows in weight matrices $ W_1 $ and $ W_2 $.
  For simplicity, bias terms are not presented.}
  \label{fig:binary_classification_neural_network}
\end{figure}
%
Then, we inferred codes for 25 thousands test set documents and we predicted their sentiment using neural network.
We conducted those experiments in two variants: with dictionary constructed only from words and with dictionary containing all words and bigrams. We call the second model paragraph vector distributed bag of n-grams (PV-DBONG).
Results are presented in~\tabref{dbong_results}.
%
\begin{table}[htb]
  \centering
    \begin{tabular}{|c|c|}
      \hline
      Model    & Error rate \\ \hline
      PV-DBOW  & 11.92\%    \\ \hline
      PV-DBONG & 9.53\%     \\ \hline
    \end{tabular}
  \caption{The performance of PV-DBONG compared to PV-DBOW}
  \label{tab:dbong_results}
\end{table}
%
As shown, using bi-grams in addition to uni-grams yields 20\% classification error reduction.

\section{Conclusions}

In this chapter we presented very simple yet effective extension to paragraph vector distributed bag of words model.
This extension can only be used for the PV-DBOW model,
since in case of PV-DM we explicitly predict center word (unigram) based on its context.
TODO: compare to~\cite{li2015learning}.
